Fact-Checking with Contextual Narratives: Leveraging Retrieval-Augmented LLMs for Social Media Analysis

We propose CRAVE (Cluster-based Retrieval Augmented Verification with Explanation); a novel framework that integrates retrieval-augmented Large Language Models (LLMs) with clustering techniques to address fact-checking challenges on social media. CRAVE automatically retrieves multimodal evidence from diverse, often contradictory, sources. Evidence is clustered into coherent narratives, and evaluated via an LLM-based judge to deliver fact-checking verdicts explained by evidence summaries. By synthesizing evidence from both text and image modalities and incorporating agent-based refinement, CRAVE ensures consistency and diversity in evidence representation. Comprehensive experiments demonstrate CRAVE's efficacy in retrieval precision, clustering quality, and judgment accuracy, showcasing its potential as a robust decision-support tool for fact-checkers.

==> d.tex <==
\begin{table*}[]
\small
\begin{tabular}{ll|llllll|llllll|llllll|llllll|}
\cline{3-26}
                                                   &   & \multicolumn{6}{l|}{Verite}                                                                                                                      & \multicolumn{6}{l|}{MMFakeb}                                                                                                                     & \multicolumn{6}{l|}{5pils}                                                                                                                       & \multicolumn{6}{l|}{NewsCLIPpings}                                                                                             \\ \cline{3-26} 
                                                   &   & \multicolumn{3}{l|}{Max}                                                          & \multicolumn{3}{l|}{Cluster}                                 & \multicolumn{3}{l|}{max}                                                          & \multicolumn{3}{l|}{cluster}                                 & \multicolumn{3}{l|}{max}                                                          & \multicolumn{3}{l|}{cluster}                                 & \multicolumn{3}{l|}{Max}                                                 & \multicolumn{3}{l|}{Cluster}                        \\ \cline{3-26} 
                                                   &   & \multicolumn{1}{l|}{O}    & \multicolumn{1}{l|}{T}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{O}    & \multicolumn{1}{l|}{T}    & F    & \multicolumn{1}{l|}{O}    & \multicolumn{1}{l|}{T}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{O}    & \multicolumn{1}{l|}{T}    & F    & \multicolumn{1}{l|}{O}    & \multicolumn{1}{l|}{T}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{O}    & \multicolumn{1}{l|}{T}    & F    & \multicolumn{1}{l|}{O} & \multicolumn{1}{l|}{T} & \multicolumn{1}{l|}{F} & \multicolumn{1}{l|}{O} & \multicolumn{1}{l|}{T} & F \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{XV}}          & A & \multicolumn{3}{l|}{0.75}                                                         & \multicolumn{3}{l|}{0.82}                                    & \multicolumn{3}{l|}{0.71}                                                         & \multicolumn{3}{l|}{0.75}                                    & \multicolumn{3}{l|}{0.89}                                                         & \multicolumn{3}{l|}{0.90}                                    & \multicolumn{3}{l|}{}                                                    & \multicolumn{3}{l|}{}                               \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & P & \multicolumn{1}{l|}{0.74} & \multicolumn{1}{l|}{0.66} & \multicolumn{1}{l|}{0.78} & \multicolumn{1}{l|}{0.81} & \multicolumn{1}{l|}{0.79} & 0.83 & \multicolumn{1}{l|}{0.68} & \multicolumn{1}{l|}{0.52} & \multicolumn{1}{l|}{0.74} & \multicolumn{1}{l|}{0.74} & \multicolumn{1}{l|}{0.72} & 0.76 & \multicolumn{1}{l|}{0.89} & \multicolumn{1}{l|}{0.91} & \multicolumn{1}{l|}{0.88} & \multicolumn{1}{l|}{0.91} & \multicolumn{1}{l|}{0.95} & 0.89 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & R & \multicolumn{1}{l|}{0.75} & \multicolumn{1}{l|}{0.54} & \multicolumn{1}{l|}{0.86} & \multicolumn{1}{l|}{0.82} & \multicolumn{1}{l|}{0.63} & 0.91 & \multicolumn{1}{l|}{0.71} & \multicolumn{1}{l|}{0.27} & \multicolumn{1}{l|}{0.89} & \multicolumn{1}{l|}{0.75} & \multicolumn{1}{l|}{0.27} & 0.96 & \multicolumn{1}{l|}{0.89} & \multicolumn{1}{l|}{0.68} & \multicolumn{1}{l|}{0.97} & \multicolumn{1}{l|}{0.90} & \multicolumn{1}{l|}{0.70} & 0.98 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & F & \multicolumn{1}{l|}{0.74} & \multicolumn{1}{l|}{0.59} & \multicolumn{1}{l|}{0.82} & \multicolumn{1}{l|}{0.81} & \multicolumn{1}{l|}{0.70} & 0.87 & \multicolumn{1}{l|}{0.68} & \multicolumn{1}{l|}{0.36} & \multicolumn{1}{l|}{0.81} & \multicolumn{1}{l|}{0.71} & \multicolumn{1}{l|}{0.39} & 0.84 & \multicolumn{1}{l|}{0.88} & \multicolumn{1}{l|}{0.78} & \multicolumn{1}{l|}{0.93} & \multicolumn{1}{l|}{0.90} & \multicolumn{1}{l|}{0.80} & 0.93 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{XV(R)}}       & A & \multicolumn{3}{l|}{0.74}                                                         & \multicolumn{3}{l|}{0.83}                                    & \multicolumn{3}{l|}{0.72}                                                         & \multicolumn{3}{l|}{0.77}                                    & \multicolumn{3}{l|}{0.89}                                                         & \multicolumn{3}{l|}{0.94}                                    & \multicolumn{3}{l|}{}                                                    & \multicolumn{3}{l|}{}                               \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & P & \multicolumn{1}{l|}{0.73} & \multicolumn{1}{l|}{0.66} & \multicolumn{1}{l|}{0.77} & \multicolumn{1}{l|}{0.84} & \multicolumn{1}{l|}{0.85} & 0.83 & \multicolumn{1}{l|}{0.71} & \multicolumn{1}{l|}{0.54} & \multicolumn{1}{l|}{0.78} & \multicolumn{1}{l|}{0.77} & \multicolumn{1}{l|}{0.79} & 0.77 & \multicolumn{1}{l|}{0.89} & \multicolumn{1}{l|}{0.85} & \multicolumn{1}{l|}{0.91} & \multicolumn{1}{l|}{0.94} & \multicolumn{1}{l|}{0.94} & 0.94 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & R & \multicolumn{1}{l|}{0.74} & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.87} & \multicolumn{1}{l|}{0.83} & \multicolumn{1}{l|}{0.62} & 0.95 & \multicolumn{1}{l|}{0.72} & \multicolumn{1}{l|}{0.43} & \multicolumn{1}{l|}{0.84} & \multicolumn{1}{l|}{0.77} & \multicolumn{1}{l|}{0.32} & 0.96 & \multicolumn{1}{l|}{0.89} & \multicolumn{1}{l|}{0.78} & \multicolumn{1}{l|}{0.94} & \multicolumn{1}{l|}{0.94} & \multicolumn{1}{l|}{0.84} & 0.98 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & F & \multicolumn{1}{l|}{0.73} & \multicolumn{1}{l|}{0.56} & \multicolumn{1}{l|}{0.82} & \multicolumn{1}{l|}{0.83} & \multicolumn{1}{l|}{0.71} & 0.88 & \multicolumn{1}{l|}{0.71} & \multicolumn{1}{l|}{0.48} & \multicolumn{1}{l|}{0.81} & \multicolumn{1}{l|}{0.74} & \multicolumn{1}{l|}{0.46} & 0.85 & \multicolumn{1}{l|}{0.89} & \multicolumn{1}{l|}{0.81} & \multicolumn{1}{l|}{0.93} & \multicolumn{1}{l|}{0.94} & \multicolumn{1}{l|}{0.89} & 0.96 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{Cluster (R)}} & A & \multicolumn{3}{l|}{0.78}                                                         & \multicolumn{3}{l|}{0.83}                                    & \multicolumn{3}{l|}{0.73}                                                         & \multicolumn{3}{l|}{0.77}                                    & \multicolumn{3}{l|}{0.91}                                                         & \multicolumn{3}{l|}{0.93}                                    & \multicolumn{3}{l|}{}                                                    & \multicolumn{3}{l|}{}                               \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & P & \multicolumn{1}{l|}{0.77} & \multicolumn{1}{l|}{0.73} & \multicolumn{1}{l|}{0.79} & \multicolumn{1}{l|}{0.83} & \multicolumn{1}{l|}{0.82} & 0.83 & \multicolumn{1}{l|}{0.71} & \multicolumn{1}{l|}{0.55} & \multicolumn{1}{l|}{0.78} & \multicolumn{1}{l|}{0.77} & \multicolumn{1}{l|}{0.76} & 0.77 & \multicolumn{1}{l|}{0.91} & \multicolumn{1}{l|}{0.82} & \multicolumn{1}{l|}{0.94} & \multicolumn{1}{l|}{0.93} & \multicolumn{1}{l|}{0.91} & 0.94 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & R & \multicolumn{1}{l|}{0.78} & \multicolumn{1}{l|}{0.52} & \multicolumn{1}{l|}{0.90} & \multicolumn{1}{l|}{0.83} & \multicolumn{1}{l|}{0.62} & 0.93 & \multicolumn{1}{l|}{0.73} & \multicolumn{1}{l|}{0.40} & \multicolumn{1}{l|}{0.87} & \multicolumn{1}{l|}{0.77} & \multicolumn{1}{l|}{0.31} & 0.96 & \multicolumn{1}{l|}{0.91} & \multicolumn{1}{l|}{0.87} & \multicolumn{1}{l|}{0.92} & \multicolumn{1}{l|}{093}  & \multicolumn{1}{l|}{0.84} & 0.97 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                             & F & \multicolumn{1}{l|}{0.76} & \multicolumn{1}{l|}{0.61} & \multicolumn{1}{l|}{0.84} & \multicolumn{1}{l|}{0.82} & \multicolumn{1}{l|}{0.71} & 0.88 & \multicolumn{1}{l|}{0.71} & \multicolumn{1}{l|}{0.46} & \multicolumn{1}{l|}{0.82} & \multicolumn{1}{l|}{0.73} & \multicolumn{1}{l|}{0.44} & 0.85 & \multicolumn{1}{l|}{0.91} & \multicolumn{1}{l|}{0.85} & \multicolumn{1}{l|}{0.94} & \multicolumn{1}{l|}{0.93} & \multicolumn{1}{l|}{0.88} & 0.95 & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  &   \\ \hline
\end{tabular}
\end{table*}
